Spatial Load Correlation in AI Data-Center-Dominated Power Systems

The proliferation of large-scale data centers introduces spatially correlated demand profiles that challenge the long-standing assumption of statistical independence of loads in power system analysis. This paper examines the emergence of such load correlations and evaluates their impact on data-center-dominated grids. Analytical derivations reveal that correlated load fluctuations amplify aggregate stochastic disturbances, reduce voltage stability margins through weakened reactive power stiffness, and degrade frequency stability margin by erosion of natural load diversity effects. Real-time digital simulation studies confirm that moderate spatial correlation in distributed data centers produces simultaneous frequency deviations and voltage fluctuations across multiple buses. The findings offer transmission system operators a physics-based perspective to interpret emerging oscillatory phenomena and establish stability planning criteria grounded in measurable load-correlation structures rather than traditional diversity assumptions.

==> merged_image.tex <==
\begin{figure}[htbp]
\centering
\begin{tikzpicture}[scale=0.75, every node/.style={scale=0.75}]

% =====================================================
% TRANSMISSION LEVEL
% =====================================================
\node[circle, draw, thick, fill=red!12, minimum size=0.9cm] (B1) at (0,5) {\scriptsize Bus 1};
\node[circle, draw, thick, fill=red!12, minimum size=0.9cm] (B2) at (3.8,5) {\scriptsize Bus 2};
\node[circle, draw, thick, fill=red!12, minimum size=0.9cm] (B3) at (7.6,5) {\scriptsize Bus 3};

\draw[very thick, red!60!black] (B1)--(B2) node[midway,above,font=\scriptsize]{230 kV};
\draw[very thick, red!60!black] (B2)--(B3) node[midway,above,font=\scriptsize]{230 kV};

\node[font=\scriptsize, text=red!70!black] at (3.8,5.75) {Transmission Level};

% =====================================================
% SUBTRANSMISSION LEVEL
% =====================================================
\foreach \x/\name in {0/Sub.1, 2.5/Sub.2, 5.1/Sub.3, 7.6/Sub.4}{
  \node[circle, draw, thick, fill=blue!18, minimum size=0.85cm] (S\x) at (\x,3.2) {\scriptsize \name};
}

\draw[thick,blue!60!black](B1)--(0,4.1);
\draw[thick,blue!60!black](B2)--(2.5,4.1)
    (B2)--(5.1,4.1);
\draw[thick,blue!60!black](B3)--(7.6,4.1);

\draw[thick,blue!70!black](0,4.1)--(S0);
\draw[thick,blue!70!black](2.5,4.1)--(S2.5);
\draw[thick,blue!70!black](5.1,4.1)--(S5.1);
\draw[thick,blue!70!black](7.6,4.1)--(S7.6);

\draw[thick,blue!40](S0)--(S2.5) node[midway,above,font=\scriptsize]{69--138 kV};
\draw[thick,blue!40](S5.1)--(S7.6) node[midway,above,font=\scriptsize]{69--138 kV};

\node[font=\scriptsize, text=blue!70!black] at (3.8,3.55) {Subtransmission Level};

% =====================================================
% DATA CENTERS + LOAD
% =====================================================

\node[rectangle, draw, thick, fill=orange!20, minimum width=2cm, minimum height=1.1cm, align=center]
(DC1) at (0,1.1) {\scriptsize\textbf{Data Center 1}\\[-2pt]\scriptsize150 MW\\[-2pt]\scriptsize AI Training};

\node[rectangle, draw, thick, fill=orange!20, minimum width=2cm, minimum height=1.1cm, align=center]
(DC2) at (2.5,1.1) {\scriptsize\textbf{Data Center 2}\\[-2pt]\scriptsize180 MW\\[-2pt]\scriptsize AI Training};

\node[rectangle, draw, thick, fill=green!15, minimum width=1.8cm, minimum height=1.1cm, align=center]
(LOAD) at (5.1,1.1) {\scriptsize Independent\\[-2pt]\scriptsize Load 50 MW};

\node[rectangle, draw, thick, fill=orange!20, minimum width=2cm, minimum height=1.1cm, align=center]
(DC3) at (7.6,1.1) {\scriptsize\textbf{Data Center 3}\\[-2pt]\scriptsize120 MW\\[-2pt]\scriptsize AI Inference};

\draw[->,thick,orange!70!black](DC1)--(S0) node[midway,left,font=\scriptsize]{$P_1$};
\draw[->,thick,orange!70!black](DC2)--(S2.5) node[midway,right,font=\scriptsize]{$P_2$};
\draw[->,thick,green!60!black](LOAD)--(S5.1) node[midway,right,font=\scriptsize]{$P_4$};
\draw[->,thick,orange!70!black](DC3)--(S7.6) node[midway,left,font=\scriptsize]{$P_3$};

% Correlation arrows
\coordinate (DC2_mid) at ($(DC2.south west)!0.55!(DC2.south east)$);

\draw[<->,thick,red!70!black,dashed]
  (DC1.south) to[bend right=18]
  node[midway,below=3pt,font=\scriptsize,text=red!70!black]{Sync'd workloads}
  (DC2_mid);

\draw[<->,thick,red!70!black,dashed]
  ($(DC2.south east)!0.52!(DC2.south west)$)
  to[bend right=16]
  node[midway,below=1.5pt,font=\scriptsize,text=red!70!black]{Correlated}
  (DC3.south);

% =====================================================
% ZOOMED-IN INSET FOR DC3
% =====================================================
\node[rectangle, draw, thick, fill=red!10,
      minimum width=3.2cm, minimum height=2.2cm,
      anchor=west] (inset) at (9.2,1.3) {};

\node[font=\scriptsize, align=center, text=black]
      at (10.8,2.25) {\scriptsize\textbf{Zoomed: Internal}\\[-2pt]\scriptsize\textbf{Local Sync Only}};

% GPU racks
\node[rectangle, draw, fill=orange!30, minimum width=1.2cm, minimum height=0.35cm]
(g1) at (9.8,1.95) {};
\node[rectangle, draw, fill=orange!30, minimum width=1.2cm, minimum height=0.35cm]
(g2) at (9.8,1.55) {};
\node at (9.8,1.25) {\scriptsize$\vdots$};
\node[rectangle, draw, fill=orange!30, minimum width=1.2cm, minimum height=0.35cm]
(gN) at (9.8,0.95) {};

% HVAC
\node[rectangle, draw, fill=cyan!25, minimum width=1.2cm, minimum height=0.4cm]
(HVAC) at (11.1,1.3) {\scriptsize HVAC};

% internal sync arrow
\draw[<->, dashed, thick, orange!80!black]
(g1.east) -- ++(0.5,0) -- ++(0,-1.0) -- (gN.east);

% Arrow from DC3 to inset
\draw[->,very thick,blue!70!black]
(DC3.east) -- (inset.west)
node[midway,above,font=\scriptsize]{\textbf{Local internal sync}};

% Internal independence annotation
\node[text=red!80!black, font=\scriptsize, align=center]
at (10.7,0.55)
{No spatial\\correlation};

\end{tikzpicture}
\caption{Correlated multi-site data centers with a zoomed-in inset showing internal synchronization within Data Center~3.}
\label{fig:zoomed_dc}
\end{figure}

